Pixel-Level Clustering Network for Unsupervised Image Segmentation

While image segmentation is crucial in various computer vision applications, such as autonomous driving, grasping, and robot navigation, annotating all objects at the pixel-level for training is nearly impossible. Therefore, the study of unsupervised image segmentation methods is essential. In this paper, we present a pixel-level clustering framework for segmenting images into regions without using ground truth annotations. The proposed framework includes feature embedding modules with an attention mechanism, a feature statistics computing module, image reconstruction, and superpixel segmentation to achieve accurate unsupervised segmentation. Additionally, we propose a training strategy that utilizes intra-consistency within each superpixel, inter-similarity/dissimilarity between neighboring superpixels, and structural similarity between images. To avoid potential over-segmentation caused by superpixel-based losses, we also propose a post-processing method. Furthermore, we present an extension of the proposed method for unsupervised semantic segmentation. We conducted experiments on three publicly available datasets (Berkeley segmentation dataset, PASCAL VOC 2012 dataset, and COCO-Stuff dataset) to demonstrate the effectiveness of the proposed framework. The experimental results show that the proposed framework outperforms previous state-of-the-art methods.

==> qualitative2.tex <==
\begin{figure}[!t] 

\begin{minipage}{0.026\linewidth}
\rotatebox[origin=c]{90}{{\footnotesize Image}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/100007.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/105053.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/353013.jpg}}
\end{minipage}
\\

\vspace{0.06cm}
\begin{minipage}{0.026\linewidth}
\rotatebox[origin=c]{90}{{\footnotesize Groundtruth}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/100007_gt.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/105053_gt.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/353013_gt.jpg}}
\end{minipage}
\\

%\vspace{0.06cm}
%\begin{minipage}{0.026\linewidth}
%\rotatebox[origin=c]{90}{{\footnotesize (a)}}
%\end{minipage}
%\begin{minipage}{0.3\linewidth}
%\centerline{\includegraphics[scale=0.156]{result_im2im/100007_1.jpg}}
%\end{minipage}
%\begin{minipage}{0.3\linewidth}
%\centerline{\includegraphics[scale=0.156]{result_im2im/105053_1.jpg}}
%\end{minipage}
%\begin{minipage}{0.3\linewidth}
%\centerline{\includegraphics[scale=0.156]{result_im2im/353013_1.jpg}}
%\end{minipage}
%\\

\vspace{0.06cm}
\begin{minipage}{0.026\linewidth}
\rotatebox[origin=c]{90}{{\footnotesize (b)}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/100007_2.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/105053_2.jpg}}
\end{minipage}
\begin{minipage}{0.3\linewidth}
\centerline{\includegraphics[scale=0.156]{result_im2im/353013_2.jpg}}
\end{minipage}

\caption{Qualitative results of the proposed model with different components. (a) The model without RTSE block and ESG loss, (b) the model with RTSE block and ESG loss}
\label{fig:result_im2im}
\end{figure}

